Robust Anomaly Detection and Backdoor Attack Detection Via Differential Privacy

Outlier detection and novelty detection are two important topics for anomaly detection. Suppose the majority of a dataset are drawn from a certain distribution, outlier detection and novelty detection both aim to detect data samples that do not fit the distribution. Outliers refer to data samples within this dataset, while novelties refer to new samples. In the meantime, backdoor poisoning attacks for machine learning models are achieved through injecting poisoning samples into the training dataset, which could be regarded as "outliers" that are intentionally added by attackers. Differential privacy has been proposed to avoid leaking any individual's information, when aggregated analysis is performed on a given dataset. It is typically achieved by adding random noise, either directly to the input dataset, or to intermediate results of the aggregation mechanism. In this paper, we demonstrate that applying differential privacy can improve the utility of outlier detection and novelty detection, with an extension to detect poisoning samples in backdoor attacks. We first present a theoretical analysis on how differential privacy helps with the detection, and then conduct extensive experiments to validate the effectiveness of differential privacy in improving outlier detection, novelty detection, and backdoor attack detection.

==> additional-results.tex <==
\subsection{Additional experiment results}
We list additional experimental results in this section. With more parameters being tested and more metrics being collected, these extensive results further validate our observations presented in the main paper body: differential privacy could improve anomaly detection and backdoor attack detection; and the higher ratio of outliers in the training data, the more noise (smaller privacy bound $\epsilon$) is needed to achieve the best improvement.


\subsubsection{Autoencoder anomaly detection}
Besides the AUPR scores presented in Table \ref{table:train_ae} for outlier detection and novelty detection using autoencoders, we present additional results with more parameters being tested in Table~\ref{table:ae_appdx_aupr}.
The observations are similar. As an intermediate step in differential privacy to bound the sensitivity, clipping itself without adding any noise is able to improve the performance of outlier detection and novelty detection. Adding various amounts of random Gaussian noise is able to further improve the utility, except when the amount of noise is too big (e.g., $\sigma=50$ and $100$) to ruin the model.
We also indicate the privacy bound $\epsilon$ as accumulated by the moments accountant mechanism in \cite{abadi2016deep}. Interestingly, many $\epsilon$ values are too big to provide any meaningful privacy guarantee, but they are still able to improve the anomaly detection performance.

\begin{table}[hpbt]
	\centering
	\small
	\tabcolsep=0.11cm
    \begin{tabular}{ |l||r|r||r|r||r|r||r|r||r|r||r|r||r| } \hline
    noise   &  \multicolumn{12}{|c|}{outlier percentage in training data $r_o$} & \multirow{3}{*}{$\epsilon$}  \\  \cline{2-13}
    scale    &  \multicolumn{2}{|c||}{$0.01\%$} & \multicolumn{2}{|c||}{$0.1\%$} & \multicolumn{2}{|c||}{$0.5 \%$} & \multicolumn{2}{|c||}{$1\%$} & \multicolumn{2}{|c||}{$5 \%$} & \multicolumn{2}{|c||}{$10\%$}  &   \\ \cline{2-13}
    $\sigma=$ & OD & ND & OD & ND & OD & ND & OD & ND & OD & ND & OD & ND & \\ \hline
     N/A  &  100 & 99.84 & 99.92 & 99.77 & 92.12 & 98.81 & 92.12 & 99.81 & 84.33 & 88.18 & 72.16 & 68.14 & $\infty$    \\ \hline
$0$ & 100 & 99.86 & 99.89 & 99.83 & 98.3 & 99.69 & 95.2 & 98.68 & 83.86 & 87.91 & 77.8 & 74.74 & $\infty$
 \\ \hline
    $0.001$  &  100&99.70  &
100 & 99.86 & 98.37 & 99.64 & 94.33 & 98.81 & 84.31 & 89.34 & 86.51 & 85.58 & $ 1.0\times 10^{10}$
 \\ \hline
    $  0.005$  & 100 & 99.87 & 99.82 & 99.78  & 98.69 & 99.7 & 95.67 & 98.87 & 91.01 & 94.3 & 79.55 & 77.04 & 
$3.9\times 10^8$
 \\ \hline
    $  0.01$  &  {\bf 100} & {\bf 99.89} & {\bf 100} & {\bf 99.97} &94.92 & 99.23  &97.08 & 99.33  &90.79 & 93.34  &85.41 & 84.07 & $9.8 \times 10^7$
 \\ \hline

    $  0.05$  &  100 & 99.85 & 99.89 & 99.79 & 97.97 & 99.55   &
96.94 & 99.34 & 88.84 & 92.54 & 75.18 & 72.09 & $2.8 \times 10^6 $
 \\ \hline

    $  0.1$  & 100 & 99.88 & 100 & 99.85 &
{\bf 98.44} & {\bf 99.66} &
93.11 & 98.21 &
92.23 & 94.21                     &
85.56 & 83.98 & $6.8 \times 10^4$
 \\ \hline

    $ 0.5$  &  100& 99.84 & 99.95 & 99.85 & 98.59 & 99.64 & {\bf 99.95} & {\bf 99.85} & 93.69 & 95.8 & 85.61 & 83.86 & 22.23
\\ \hline
    $  1$  &  100 & 99.81  &100 & 99.78 &98.28 & 99.67 &95.8 & 99.0   &94.92 & 96.87 &81.87 & 80.12  & 3.09
\\ \hline

    $  5$  &  100 & 99.49 & 99.87 & 99.49 & 98.51 & 99.52 &
96.5 & 98.78   &
{\bf 96.78} & {\bf 98.04} &
95.25 & 95.41 &  0.44
\\ \hline
$ 10$  & 97.62 & 97.61 & 90.24 & 97.77 & 91.88 & 98.2  &97.5 & 99.12  &96.6 & 98.2  & {\bf 97.07} & {\bf 97.46}  &  0.25
\\ \hline
\multicolumn{14}{|c|}{{\sf Below $\sigma$ value is too big such that the model does not converge well in training.}} \\ \hline
$  50$  &  54.19 & 90.46 & 65.94 & 92.13 & 70.34 & 90.8 & 78.34 & 91.19 & 86.58 & 91.59 & 88.49 & 90.27 & 0.19
\\ \hline
$  100$  &  56.08 & 87.2 & 47.22 & 70.57 & 71.95 & 90.8 & 4.23 & 10.73 & 80.58 & 86.94 & 89.26 & 90.68 & 0.19
\\ \hline
    \end{tabular}
\caption{{AUPR scores for autoencoder outlier detection (OD) and novelty detection (ND)}. }
\label{table:ae_appdx_aupr}
\end{table}

Besides AUPR scores, we further present AUROC scores in Table~\ref{table:ae_appdx_auroc} for the same set of experiments. Autoencoders, as validated by many previous works (\cite{mirsky2018kitsune,gottschlich2017autoperf}), present great effectiveness in detecting outliers and novelties, especially when the outlier ratio in training dataset is slow (e.g., below $1\%$). Although not as obvious as AUPR scores, the improvements brought by differential privacy follow a similar trend, where the improvement is more significant with larger noise (smaller $\epsilon$) being applied to models trained with more outliers.

\begin{table}[hpbt]
	\centering
	\small
	\tabcolsep=0.11cm
    \begin{tabular}{ |l||r|r||r|r||r|r||r|r||r|r||r|r||r| } \hline
    noise   &  \multicolumn{12}{|c|}{outlier percentage in training data $r_o$} & \multirow{3}{*}{$\epsilon$}  \\  \cline{2-13}
    scale    &  \multicolumn{2}{|c||}{$0.01\%$} & \multicolumn{2}{|c||}{$0.1\%$} & \multicolumn{2}{|c||}{$0.5 \%$} & \multicolumn{2}{|c||}{$1\%$} & \multicolumn{2}{|c||}{$5 \%$} & \multicolumn{2}{|c||}{$10\%$}  &   \\ \cline{2-13}
    $\sigma=$ & OD & ND & OD & ND & OD & ND & OD & ND & OD & ND & OD & ND & \\ \hline
N/A & 100 & 99.97 & 100 & 99.95 & 99.81 & 99.79 & 99.17 & 99.07 & 97.3 & 97.4 & 89.46 & 89.2 & $\infty$  \\ \hline
0 & 100 & 99.97 & 100 & 99.97 & 99.96 & 99.93 & 99.7 & 99.77 & 97.36 & 97.52 & 92.39 & 92.35 & $\infty$  \\ \hline
0.001 & 100 & 99.93 & 100 & 99.97 & 99.89 & 99.84 & 99.79 & 99.82 & 97.37 & 97.63 & 96.26 & 96.72 & $1.0\times 10^{10}$  \\ \hline
0.005 & 100 & 99.96 & 100 & 99.95 & 99.92 & 96.09 & 99.81 & 99.83 & 98.73 & 98.91 & 93.62 & 93.82 & $3.9\times 10^{8}$  \\ \hline
0.01 & 100 & 99.97 & 100 & 99.97 & 99.8 & 99.87 & 99.89 & 99.9 & 98.39 & 98.5 & 96.02 & 96.4 & $9.8\times 10^{7}$  \\ \hline
0.05 & 100 & 99.97 & 100 & 99.96 & 99.9 & 99.93 & 99.87 & 99.9 & 97.55 & 97.81 & 90.91 & 90.87 & $2.8\times 10^{6}$  \\ \hline
0.1 & 100 & 99.97 & 100 & 99.97 & 99.87 & 99.9 & 99.58 & 99.71 & 98.77 & 98.82 & 96.16 & 96.46 & $6.8\times 10^{4}$  \\ \hline
0.5 & 100 & 99.96 & 100 & 99.97 & 99.9 & 99.91 & 99.77 & 99.85 & 99.13 & 99.25 & 95.96 & 96.25 & 22.23  \\ \hline
1 & 100 & 99.95 & 100 & 99.94 & 99.91 & 99.94 & 99.74 & 99.81 & 99.31 & 99.44 & 94.66 & 94.95 & 3.09  \\ \hline
5 & 100 & 99.81 & 100 & 99.85 & 99.96 & 99.93 & 99.52 & 99.5 & 99.07 & 99.32 & 98.49 & 98.74 & 0.44  \\ \hline
10 & 100 & 99 & 99.86 & 99.25 & 99.14 & 99.93 & 99.68 & 99.79 & 98.72 & 99.29 & 98.9 & 99.27 & 0.25  \\ \hline
\multicolumn{14}{|c|}{{\sf Below $\sigma$ value is too big such that the model does not converge well in training.}} \\ \hline
50 & 99.99 & 96.11 & 94.8 & 96.41 & 92.96 & 96.13 & 94.15 & 96.29 & 7.03 & 5.95 & 93.83 & 95.61 & 0.19  \\ \hline
100 & 99.73 & 94.7 & 82.64 & 87.29 & 93.51 & 99.22 & 31.77 & 30.91 & 94.47 & 96.08 & 94.62 & 96.09 & 0.19  \\ \hline
    \end{tabular}
\caption{{AUROC scores for autoencoder outlier detection (OD) and novelty detection (ND)}. }
\label{table:ae_appdx_auroc}
\end{table}

\subsubsection{Improvements over DeepLog}
To compare the differentially private models with DeepLog, we utilize the same anomaly detection criteria, i.e., Top-\textit{k} based anomaly detection as what's presented in \cite{du2017deeplog}. Nevertheless, as a direct extension of the idea in measuring model loss for anomaly detection, we also tested the classification probability as one type of threshold for anomaly detection. 
In particular, if an actual system log entry is predicted with a probability lower than some threshold $T_p$, we treat this log entry as a detected anomaly.
While the baseline DeepLog results are not as good as the Top-\textit{k} based detection, we show that similarly, differential privacy is able to significantly reduce the number of false negatives, without introducing too many new false positives.

\Paragraph{Probability-based detection.}
As a preliminary result, we use probability-based anomaly detection to demonstrate the effectiveness of differential privacy noise in reducing \fn. Table~\ref{table:prob} shows \fn and \fp for DeepLog and DeepLog+DP with increasing noise levels, under different probability thresholds $T_p$. It is clear that differential privacy noise could effectively reduce \fn, and the larger noise being added, the more false negatives are reduced. We also note that when $\sigma=0.25$, the privacy bound $\epsilon=90.5$. It is often thought that a privacy bound $\epsilon>20$ is completely useless in terms of protecting privacy. Here we indicate that a small amount of noise may be enough to reduce \fn. Although more false positives are incurred because of differential privacy noise, the drop in \tpr is negligible, considering the large volume of normal data. For example, when $T_p=2 \times 10^{-6}$ and $\sigma=1$, the \fn drop from 1261 to 183 indicates a \tnr increase of 8\% ($91.7\% \to 98.8\%$), while the \fp increase from 2291 to 3734 only shows a \tpr decrease of 0.3\% ($99.59\% \to 99.32\%$).

\begin{table}[hbt]
% \vspace{-1mm}
	\centering
	\small
% 	\tabcolsep=0.12cm
    \begin{tabular}{ |l|r|r|r|r|r| } \hline
    Probability & {DeepLog}  &  \multicolumn{4}{|c|}{DeepLog+DP (\fn/\fp)}  \\  \cline{3-6}
    threshold {$T_p$}    & \fn/\fp & $\sigma=0.25$ & $\sigma=1$ & $\sigma=1.5$ & $\sigma=2$   \\ \hline
%    $1e-4$  & 89/5855 &  1/19614 & 0/13672 & 0/25080  &  1/22967   \\ \hline
    $10^{-5}$  &   573/3596  &  7/14268 & 0/6059 &1/8213   &   1/9187   \\ \hline
    $2\times 10^{-6}$  &  1261/2291 & 208/4756  & 183/3734 &1/5718   &  1/6317 \\ \hline
    $10^{-6}$  &  1468/2068 & 410/3759 & 190/3552 & 2/4002   &  1/6093 \\ \hline
    \end{tabular}
	\caption{{Probability-based anomaly detection results}. }
	\label{table:prob}
\end{table}

\begin{table*}[htb]
	\centering
	\tabcolsep=0.12cm
    \begin{tabular}{ |l|r|r|r|r|r|r|r|r|r| } \hline
     & \multirow{ 2}{*}{DeepLog}  &  \multicolumn{8}{|c|}{DeepLog+DP}  \\  \cline{3-10}
     &  & $\sigma$=$0.25$ & $\sigma$=$0.5$ & $\sigma$=$0.75$ & $\sigma$=$1.0$ & $\sigma$=$1.25$ & $\sigma$=$1.5$ & $\sigma$=$1.75$  & $\sigma$=$2.0$   \\ \hline
    AUROC score & 0.9993   & 0.9997  & 0.9997 & 0.9997  & 0.9998 & 0.9993  & 0.9994 & 0.9989 & 0.9985 \\ \hline
    privacy bound $\epsilon$ & 0  & 90.45  & 6.21 & 1.86   &  0.96 & 0.61 & 0.42 & 0.31 & 0.25 \\ \hline
    \end{tabular}
	\caption{{AUROC score comparison and privacy bound $\epsilon$}. }
	\label{table:auc}
\end{table*}

\paragraph{AUROC score}
To evaluate the overall performance of DeepLog+DP compared with DeepLog under different thresholds,
we further compute the AUROC score of DeepLog and DeepLog+DP with different noise scale $\sigma$.
% \auc stands for \textit{Area under curve (\auc) score}, which is the area under 
% \textit{receiver operating characteristic (ROC) curve}, where the x axis is the \fpr while the y axis denotes the \tpr. Clearly, the lower the \fpr and the higher the \tpr, the bigger the area under ROC curve, and hence the larger the \auc score.
As shown in Table~\ref{table:auc}, DeepLog already achieves excellent AUROC score, considering the large amount of normal data and the significantly fewer anomalies. However, an adequate amount of differential privacy noise is still able to improve the performance. 

\paragraph{Privacy bound $\epsilon$}
Table~\ref{table:auc} also indicates the privacy bound $\epsilon$. Note that $\epsilon<10$ is often considered as usable and $\epsilon<1$ is a tight bound that well protects privacy. Considering all the cases, $\sigma=1$ gives the best anomaly detection utility as well as a tight privacy bound to protect training data privacy.

\subsubsection{Backdoor attack detection}
In this section, we evaluate more parameters for the experiment set up described in Section~\ref{sec:exp-backdoor} {BACKDOOR ATTACK DETECTION}, and measure  \textit{benign accuracy}, \textit{success rate}, AUPR score and AUROC score as explained in Section~\ref{sec:exp-backdoor} for each experiment setting.
Similar as the observations in Section~\ref{sec:exp-backdoor}, a differentially private trained machine learning model is naturally more robust to backdoor attacks. The evidence is that the benign accuracy (Table \ref{table:train_bk_benign_appdx}) is affected little by differential privacy except when the noise scale is too big to ruin the model parameters, compared with the significant downgrade (e.g., 98.1\% to 0.3\%) in backdoor success rate (Table \ref{table:train_bk_success_appdx}). Also, as shown in Table \ref{table:bk_aupr_appdx} and Table \ref{table:bk_auroc_appdx}, measuring model loss to detect poisoning examples could be useful when the poisoning ratio is low. Nevertheless, applying differential privacy is able to significantly improve the detection performance for a poisoning ratio as high as $45\%$.

\begin{table}[hpbt]
	\centering
	\small
    \begin{tabular}{ |l|r|r|r|r|r|r|r|r|r| } \hline
   noise scale  & \multicolumn{8}{c|}{poisoning ratio in training data $r_p$} & \multirow{2}{*}{$\epsilon$} \\ \cline{2-9}
   $\sigma$ & 0.005 & 0.01 & 0.05 & 0.1 & 0.2 & 0.3 & 0.4 & 0.45 &   \\ \hline
N/A & 98.93 & 99.03 & 98.95 & 99.11 & 98.94 & 99.06 & 99.05 & 98.97 & $\infty$  \\ \hline
0 & 97.66 & 97.21 & 97.84 & 97.46 & 96.97 & 96.32 & 93.61 & 92.4 & $\infty$ \\ \hline
0.001 & 97.5 & 97.52 & 97.72 & 97.29 & 97.47 & 96.69 & 94.16 & 90.41 & $9.9\times 10^{9}$ \\ \hline
0.005 & 97.57 & 97.55 & 97.46 & 97.75 & 97.36 & 96.5 & 93.96 & 91.25 & $3.9\times 10^{8}$ \\ \hline
0.01 & 97.51 & 97.61 & 97.4 & 97.55 & 97.27 & 97.07 & 94.77 & 92.82 & $9.8\times 10^{7}$ \\ \hline
0.05 & 97.42 & 97.87 & 97.8 & 97.72 & 97.69 & 96.37 & 94.19 & 93.28 & 2830766.11 \\ \hline
0.1 & 97.55 & 97.84 & 97.7 & 97.34 & 97.29 & 96.91 & 94.11 & 91.36 & 67915.88 \\ \hline
0.5 & 97.56 & 97.29 & 97.28 & 97.37 & 97.13 & 96.55 & 95.19 & 86.37 & 22.23 \\ \hline
1 & 96.94 & 96.95 & 96.96 & 96.53 & 96.27 & 95.78 & 91.65 & 83.16 & 3.09 \\ \hline
2 & 93.76 & 93.39 & 92.16 & 93.22 & 92.77 & 92.4 & 87.61 & 81.24 & 1.18 \\ \hline
\multicolumn{10}{|c|}{{\sf Below noise level $\sigma$ could be too high.}} \\ \hline
3 & 89.85 & 89.5 & 91.12 & 90.92 & 89.35 & 89.81 & 85.42 & 76.51 & 0.75 \\ \hline
5 & 80.51 & 79.57 & 80.49 & 80.28 & 79.19 & 77.95 & 57.5 & 61.64 & 0.44 \\ \hline
10 & 17.32 & 19.82 & 20.31 & 12.07 & 11.34 & 11.43 & 11.15 & 11.11 & 0.25 \\ \hline
\end{tabular}
\caption{{Benign accuracy of models trained on datasets with different poisoning ratio $r_p$. The more noise being added, the more utility is affected.}}
\label{table:train_bk_benign_appdx}
% 	\tabcolsep=0.11cm
\end{table}



\begin{table}[hpbt]
	\centering
	\small
    \begin{tabular}{ |l|r|r|r|r|r|r|r|r|r| } \hline
   noise scale  & \multicolumn{8}{c|}{poisoning ratio in training data $r_p$} & \multirow{2}{*}{$\epsilon$} \\ \cline{2-9}
   $\sigma$ & 0.005 & 0.01 & 0.05 & 0.1 & 0.2 & 0.3 & 0.4 & 0.45 &   \\ \hline
N/A & 47.85 & 90.96 & 97.12 & 98.1 & 98.46 & 98.91 & 98.92 & 98.79 & $\infty$ \\ \hline
0 & 0.23 & 0.29 & 0.35 & 0.3 & 0.47 & 0.74 & 68.1 & 72.02 & $\infty$ \\ \hline
0.001 & 0.21 & 0.22 & 0.25 & 0.37 & 0.42 & 0.85 & 35.83 & 19.01 & $9.9\times 10^{9}$ \\ \hline
0.005 & 0.17 & 0.2 & 0.28 & 0.3 & 0.35 & 35.54 & 50.28 & 83.94 &  $3.9\times 10^{8}$ \\ \hline
0.01 & 0.25 & 0.24 & 0.34 & 0.31 & 0.42 & 0.56 & 93.64 & 15.25 & $9.8\times 10^{7}$ \\ \hline
0.05 & 0.24 & 0.25 & 0.37 & 0.3 & 0.37 & 18.55 & 82.15 & 4.53 & 2830766.11 \\ \hline
0.1 & 0.25 & 0.18 & 0.28 & 0.39 & 0.47 & 0.71 & 82.23 & 59.57 & 67915.88 \\ \hline
0.5 & 0.26 & 0.23 & 0.29 & 0.35 & 0.37 & 0.81 & 1.63 & 74.15 &  22.23 \\ \hline
1 & 0.28 & 0.3 & 0.45 & 0.5 & 0.63 & 1.09 & 44.12 & 67.44 & 3.09 \\ \hline
2 & 0.74 & 0.68 & 1.07 & 1.1 & 1.4 & 2.67 & 5.95 & 71.48 & 1.18 \\ \hline
\multicolumn{10}{|c|}{{\sf Below noise level $\sigma$ could be too high.}} \\ \hline
3 & 0.96 & 1.22 & 1.1 & 1.59 & 2.69 & 2.66 & 6.02 & 20.38 & 0.75 \\ \hline
5 & 2.01 & 1.6 & 2.44 & 3.47 & 2.68 & 8.15 & 13.78 & 19.91 & 0.44 \\ \hline
10 & 9.93 & 10.3 & 10.03 & 9.08 & 9.68 & 9.33 & 10.14 & 9.77 & 0.25 \\ \hline
\end{tabular}
\caption{{Backdoor attack success rate of models trained on datasets with different poisoning ratio $r_p$. The success rate is significantly reduced for models trained with differential privacy.}}
\label{table:train_bk_success_appdx}
% 	\tabcolsep=0.11cm
\end{table}


\begin{table}[hpbt]
	\centering
	\small
    \begin{tabular}{ |l|r|r|r|r|r|r|r|r|r| } \hline
   noise scale  & \multicolumn{8}{c|}{poisoning ratio in training data $r_p$} & \multirow{2}{*}{$\epsilon$} \\ \cline{2-9}
   $\sigma$ & 0.005 & 0.01 & 0.05 & 0.1 & 0.2 & 0.3 & 0.4 & 0.45 &  \\ \hline
N/A & 73.01 & 27.02 & 14.85 & 17.63 & 24.9 & 36.42 & 42.16 & 45.85 & $\infty$ \\ \hline
0 & 91.22 & 92.11 & 95.33 & 95.46 & 95.9 & 96.55 & 62.57 & 60.33 & $\infty$  \\ \hline
0.001 & 91.52 & 93.36 & 94.61 & 95.98 & 96.95 & 96.05 & 78.53 & 86.9 & $9.9\times 10^{9}$ \\ \hline
0.005 & 92.64 & 94.04 & 94.76 & 95.45 & 96.98 & 79.1 & 72.73 & 52.07  & $3.9\times 10^{8}$ \\ \hline
0.01 & 92.24 & 94.03 & 93.4 & 95.76 & 96.69 & 96.22 & 47.08 & 90.77  & $9.8\times 10^{7}$ \\ \hline
0.05 & 90.76 & 95.11 & 95.09 & 95.54 & 96.35 & 87.28 & 49.82 & 93.72  & 2830766.11 \\ \hline
0.1 & 92.16 & 94.85 & 95.33 & 95.28 & 96.4 & 96.67 & 51 & 65.9  & 67915.9 \\ \hline
0.5 & 92.76 & 93.4 & 94.5 & 94.93 & 95.74 & 95.88 & 95.96 & 54.99  &  22.23 \\ \hline
1 & 88.67 & 90.31 & 94.77 & 94.46 & 96.03 & 94.67 & 72.99 & 56.35  & 3.09 \\ \hline
2 & 65.01 & 78.51 & 80.76 & 87.54 & 88.76 & 87.63 & 86.75 & 51.41  & 1.18 \\ \hline
\multicolumn{10}{|c|}{{\sf Below noise level $\sigma$ could be too high.}} \\ \hline
3 & 29.31 & 51.37 & 78.25 & 81 & 79.83 & 81.56 & 84.46 & 71.62  & 0.75 \\ \hline
5 & 6.4 & 17.39 & 58.66 & 58.88 & 61.8 & 69.19 & 64.27 & 61.58  & 0.44 \\ \hline
10 & 0.8 & 2 & 10.12 & 10.88 & 20.32 & 30.89 & 40.92 & 45.17  & 0.25 \\ \hline
\end{tabular}
\caption{{AUPR scores for backdoor attack detection. Applying differential privacy significantly improves the results.}}
\label{table:bk_aupr_appdx}
% 	\tabcolsep=0.11cm
\end{table}

\begin{table}[htbp]
	\centering
	\small
    \begin{tabular}{ |l|r|r|r|r|r|r|r|r|r| } \hline
   noise scale  & \multicolumn{8}{c|}{poisoning ratio in training data $r_p$} & \multirow{2}{*}{$\epsilon$} \\ \cline{2-9}
   $\sigma$ & 0.005 & 0.01 & 0.05 & 0.1 & 0.2 & 0.3 & 0.4 & 0.45 &  \\ \hline

N/A&99.26&95.23&78.88&67.72&59.47&60.9&55.33&52.73& $\infty$  \\ \hline
0&99.92 & 99.88&99.79 & 99.72&99.51 & 99.31&70.24 & 62.88 & $\infty$ 	\\ \hline
0.001&99.91 & 99.88&99.79 & 99.72&99.62 & 99.27&81.27 & 88.1 & $9.9\times 10^{9}$  \\ \hline
0.005&99.9 & 99.93&99.79 & 99.75&99.63 & 84.51&75.12 & 60.21 & $3.9\times 10^{8}$  \\ \hline
0.01&99.92 & 99.92&99.74 & 99.74&99.61 & 99.3&61.83 & 93.78& $9.8\times 10^{7}$  \\ \hline
0.05 & 99.9 & 99.94&99.83 & 99.73&99.59 & 90.67&58.03 & 97.12 & 2830766.11  \\ \hline
0.1&99.93 & 99.93&99.82 & 99.69&99.55 & 99.37&59.71 & 65.55 & 67915.88  \\ \hline
0.5&99.95 & 99.92&99.76 & 99.68&99.5 & 99.23&98.68 & 58.44 &   22.23 \\ \hline
1&99.86 & 99.84&99.76 & 99.61&99.43 & 98.87&75.7 & 63.94&3.09 \\ \hline
2&99.64 & 99.64&98.97 & 98.86&98.21 & 97.13 & 94.82 & 57.81&1.18  \\ \hline
\multicolumn{10}{|c|}{{\sf Below noise level $\sigma$ could be too high.}} \\ \hline
3&98.68 & 98.92&98.68 & 98.17&96.73 & 95.92&93.86 & 81.22&0.75 \\ \hline
5&95.74 & 96.13&96.38 & 94.42&92.22 & 89.52&77.77 & 73.11&0.44  \\ \hline
10&56.77 & 60.49&61.2 & 53.11&51.05 & 51.33 & 51.19 & 50.35 & 0.25  \\ \hline
\end{tabular}
\caption{{AUROC scores for backdoor attack detection. It shows that measuring model loss for poisoning samples detection could be effective when the poisoning ratio is low. Differential privacy improves the performance in all cases, except when the noise scale is too big to ruin the model parameters.}}
\label{table:bk_auroc_appdx}
% 	\tabcolsep=0.11cm
\end{table}




   


==> previous.tex <==


\begin{abstract}
Differential privacy has been proposed to avoid leaking individual's information while performing aggregated analysis on a given dataset. It is typically achieved by adding random noise, either directly to the input dataset, or to intermediate results of the aggregation mechanism. The added noise inevitably brings utility downgrade as shown by many previous work, despite its ability to hide individual data. In this paper, we demonstrate that applying differential privacy could surprisingly improve the performance of a type of anomaly detection approach: zero-positive anomaly detection. Specifically, our experimental results indicate that the number of false negatives are significantly reduced, without introducing many false positives.
%Abstracts must be a single paragraph, ideally between 4--6 sentences long.
%Gross violations will trigger corrections at the camera-ready phase.
\end{abstract}

\section{Introduction}
\label{intro}
The successful deployment of various data analysis techniques has highlighted the importance of comprehensive data, but also raised privacy concerns. Given an input dataset and the statistical ouput calculated from this dataset, differential privacy aims to ``hide'' certain input data from the output. The general idea is that, by looking at the statistical results calculated from input data, one can not tell whether the input data contains a certain record or not.
The way of applying differential privacy is to add random noise to the input data or the data analysis procedure, such that the output difference caused by the input difference could be hidden by noise.
Intuitively, the statistical results with differential privacy applied will become less accurate. Previous work on deep learning with differential privacy has also shown evident utility drop~\cite{abadi2016deep}.
However, it is also noted that differential privacy has the potential to prevent overfitting~\cite{pnml}, because of its ability to generalize from data~\cite{nissim2015generalization}, without depending on any single record.
Inspired by this observation, we apply differential privacy to a type of anomaly detection approach: zero-positive anomaly detection, which shows significant utility improvement.

Zero-positive anomaly detection only requires normal data for training, without the need of any ``positives''. The model training process is to extract the distribution or common information of the training data. In detection, for each data record, the model output could be checked against a threshold to detect whether the record is an anomaly (a positive).
For example, a LSTM model could be trained on normal system command sequences, e.g., \textit{login, passwd, web, mail, ssh}, as a supervised classification task, to output the probability distribution of the next command following a given input history. For anomaly detection of real-time system commands, we could simply check if the executed system command has a predicted probability lower than the threshold, given its history.
Note that anomaly detection is sometimes referred as outlier detection, where rare events that differ from the majority are considered as anomalous. In the case of zero-positive anomaly detection, we want the model \textit{not to} learn from outliers, i.e., not to overfit to rare data records. A false negative in anomaly detection means that a true anomaly is not detected. We apply differential privacy to the model training process, to prevent it from learning outliers. The anomaly detection results show significantly reduced false negatives, validating the assumption. 
Moreover, the extra false positives being introduced are mostly negligible, and the overall utility is improved.

\section{Preliminary}
\subsection{Differential privacy}
\label{sec:dp_pre}
Given an input dataset and an aggregation mechanism, {\em differential privacy}~\cite{differential} aims to output requested aggregation results, without revealing any individual data record.
Formally, differential privacy is defined as below:

\begin{definition}{Differential privacy.}
Suppose a mechanism $\mathcal{M}$ maps a data domain $\mathcal{D}$ to a region $\mathcal{R}$. $\mathcal{M}$ is said to be \{$\epsilon$, $\delta$\}-differentially private if for any adjacent datasets $d$, $d'$ in $\mathcal{D}$, and any subset of outputs $S$ $\in$ $\mathcal{R}$, there exists
$$
Pr[\mathcal{M}(d) \in S] \le e^{\epsilon} Pr[\mathcal{M}(d') \in S] + \delta,
$$
\end{definition} 
where $\epsilon$ stands for the privacy bound, and $\delta$ stands for the probability to break this bound.
The \textit{adjacent} datasets $d$, $d'$ could be understood as two database tables, where only one row differs. Differential privacy guarantees that the difference between $d$ and $d'$ are not revealed through inspecting the outputs $\mathcal{M}(d)$ and $\mathcal{M}(d')$.
Clearly, the closer $\epsilon$ is to $0$, the more indistinguishable $\mathcal{M}(d)$ and $\mathcal{M}(d')$ are, and hence the better the privacy guarantee. The maximum allowed difference for $\mathcal{M}(d)$ and $\mathcal{M}(d')$
%, if $d$ and $d'$ differ by one record, 
is referred as \textit{sensitivity}. 
In machine learning applications, 
$\mathcal{D}$ is the domain for training data, $\mathcal{R}$ is the domain for model parameters, and
$\mathcal{M}$ could be understood as the training process.
% Differential privacy is typically enforced through
% adding random noise 
% (e.g., drawn from some Gaussian distribution) to $\specialmath{M}$~\cite{abadi2016deep}.
% which ensures that the existence of a single record in the training data cannot be inferred from the model parameters.



% %Applying differential privacy is typically 
% Differential privacy is typically enforced through
% adding random noise 
% (e.g., drawn from some Gaussian distribution) to $\specialmath{M}$~\cite{abadi2016deep}.
% %which ensures that the existence of a single record in the training data cannot be inferred from the model parameters.


\subsection{Anomaly detection}
\label{sec:ad_pre}
We use LSTM models trained on discrete sequences to demonstrate our work.
In particular, discrete sequence data
are a type of time series data where each data point is a discrete
value from a fixed vocabulary set. Such data are widely
generated by many applications, for example, operating system call
sequences and phone APP API call sequences.
We could train a LSTM model on normal system execution sequences as a supervised classification task. Specifically, given a history sequence data as input, the LSTM model could be trained to predict the next system key to appear. With an output softmax layer,
the model prediction is a probability distribution over all possible keys, indicating
the likelihood of each key being the next data point. An example is
shown in Figure~\ref{fig:lstm_seq_ad}. To detect if an execution key is normal
or not, the anomaly detection model takes its history as input, and
outputs a probability distribution over all possible keys. The execution key to be checked is detected normal if the model assigns
it a probability higher than some threshold, otherwise abnormal,
indicating that something unlikely to happen has happened. As in
Figure~\ref{fig:lstm_seq_ad}, given a history sequence of \textit{A, B, C}, the prediction could
be \textit{\{D: 0.8, A: 0.2, B: 0, ...\}}, showing that the probability of having D
after the input history is 80\%, while the probability of having A is
20\%. Suppose the threshold to be detected as an anomaly is 0.1\%.
The execution key \circled{?} at time t is normal if it is D or A (having
probability higher than 0.1\%), and abnormal if it is one of the other
keys such as B, C (having probability lower than 0.1\%).

\begin{figure}[h!]
	\centering{
		\includegraphics[width=\linewidth]{seq_intro.pdf}
	}
	\caption{An example of LSTM anomaly detection on discrete sequence data.}
	\label{fig:lstm_seq_ad}
\end{figure}

\section{Applying differential privacy to anomaly detection}
In this section, we show the procedure to improve anomaly detection results using differential privacy (DP). % and present the experimental results.
For the baseline model, we use DeepLog~\cite{du2017deeplog}, which performs zero-positive system log anomaly detection using LSTM. It trains a LSTM model on normal execution system log sequences, leveraging the fact that hidden execution paths written in source code restrict the possibilities of how one system log follows another. For detection, DeepLog accepts a history log sequence as input, and outputs the next system log that may happen. It further compares the model generated log with the system generated one, and detects the real system log as anomalous if it's unlikely to happen in prediction.
Note that system log messages are textual logs, e.g., \textit{``Transaction A finished on server B.''}. Before applying LSTM, a log parsing step first parses each log message into its corresponding log printing statement in the source code, e.g., \textit{``print('Transaction \%s finished on server \%s.''\%(x,y))"}. Since there are only a constant number of log printing statements in the source code, each one could be mapped to a discrete value from a fixed vocabulary set. LSTM could then be applied to the discrete sequences parsed from system logs. Further anomaly detection works as in Section~\ref{sec:ad_pre}.

For DP, we apply the method dedicated for deep learning presented in~\cite{abadi2016deep}.
Deep learning model training is to minimize a loss function, through numerous stochastic gradient descent (SGD) steps. The differentially private SGD algorithm works as follows. At each SGD step, the per-example gradient is computed for a randomly selected set of training examples. Each gradient is clipped with the same clipping bound $C$, which is the sensitivity for DP. 
The clipped per-example gradients are then summed together with random Gaussian noise having standard deviation $\sigma$. 
%(could be calculated using $C$, $\epsilon$ and $\delta$). 
The summed result is further averaged for model parameter update.
Intuitively, the added random noise is to hide the difference of a single record from the output, i.e., model parameters. As a result, the contribution of rare training examples will be hidden by random noise, resulting a more generalized model that does not overfit to outliers.
% The way of applying DP to deep learning is to add noise to each SGD step. 
% Noise scale $\sigma$ is the standard deviation of the added Gaussian random noise. 
% Differential privacy could be applied to deep learning following~\cite{abadi2016deep}, which adds random Gaussian noise to the calculated gradients at each stochastic gradient descent iteration.
% It uses a clipping bound $C$ to bound the per-example gradient computed for a number of randomly selected training examples. The bound is further used as the sensitivity, which is the maximum difference between $\specialmath{M}(d)$ and $\specialmath{M}(d')$. A random Gaussian noise with standard deviation $\sigma$ (computed using $C$, $\epsilon$, and $\delta$) is added to the sum of the clipped per-example gradients, before averaging for gradient descent.

%In general, ML model parameters could be viewed as the statistical output calculated from input data. Note that model parameters are accumulated through iterations of gradients update. To hide a single record from the output model parameters, a typical way is to first clip the norm of gradients calculated from each record, and then add noise that is  big enough to hide the bounded updates incurred by a single record.
%as big as the clipping bound.



\section{Evaluation}
\paragraph{Dataset.}
We use Hadoop file system (HDFS) log dataset~\cite{hdfslog} for our evaluation,
which is generated through running Hadoop map-reduce jobs for 48 hours on 203 Amazon EC2 nodes.
It contains various types of anomalies labeled by domain experts, details of which could be found in~\cite{xu2009detecting}.
This dataset contains over 11 million log entries, which could be further grouped into $575,059$ block sessions by the block identifier each log has. Different blocks could be understood as concurrent threads, while the logs having the same block identifier are executed sequentially. Over the past decade this log dataset has been extensively used for research in system log parsing and anomaly detection~\cite{xu2009detecting, lou2010mining, du2016spell, du2017deeplog}.
The state-of-the-art anomaly detection results are achieved by DeepLog~\cite{du2017deeplog}, which we use as the baseline model in this work.
Note that the labels are only provided at the block session level, i.e., each normal/abnormal label is associated with a block identifier, rather than a log entry. 
As in DeepLog, our training dataset contains $4,855$ normal block sessions, while the test dataset includes $553,366$ normal sessions and $16,838$ abnormal sessions.
For detection, we say a log session is detected as normal if each log entry in this session is normal; and abnormal if at least one log entry in this session is detected as abnormal.

\paragraph{Anomaly detection metrics.}
We explain the  criteria and metrics used to evaluate the anomaly detection performance under different settings.
Suppose a LSTM model is trained on normal discrete sequences, which learns to predict the next discrete value given its hisotry. In detection, the LSTM model predicts a probability distribution on all possible values that may appear at a given time step. The real executed value is detected as abnormal if it's \textit{unlikely} to happen based on LSTM prediction.
To judge whether a value is unlikely to happen, a naive way is presented in Section~\ref{sec:ad_pre}. It compares the predicted probability of the given value (e.g., \circled{?} in Figure~\ref{fig:lstm_seq_ad}) with a probability threshold $T_p$, and detects \circled{?} as abnormal if the probability is lower than $T_p$. We call this \textit{probability-based detection}.
The criteria presented in DeepLog~\cite{du2017deeplog} is to first sort the predicted values based on the assigned probabilities, e.g., for the example in Figure~\ref{fig:lstm_seq_ad}, the order would be \textit{D,A,B,C,...}. The given value to detect is checked against the the sorted top k predictions, and is detected as abnormal if it's not one of them.
We refer this as \textit{top-k detection}. For anomaly detection metrics, we want to highlight that applying DP significantly reduces false negatives, while having mostly negligible effect on false positives. Therefore, we'll focus on the comparison over the number of false positives and false negatives, while also presenting other measurements that indicate the overall detection performance. 
The following metrics are used for evaluation: \fp, \fn, \tpr, \tnr, \fpr which could be found in~\cite{wiki:fpfn}, and \pre, \rec, \fm which are explained in~\cite{wiki:fm}.
% We use \fp to represent number of false positives, and \fn as number of false negatives; \tp is the true anomalies being detected and \tn is the number of true negatives. \tpr is the true positive rate which equals \tp/(\tp+\fn). \tnr is the true negative rate and is \tn/(\tn+\fp), while \fpr=\fp/(\tn+\fp) is the false positive rate. Finally, as an overall measurement for highly unbalanced classes, we use \fm, which is calculated as 2*(\pre*\rec)/(\pre+\rec), where \pre = \tp/(\tp+\fp) indicating how many anomalies are true among all detected anomalies, while \rec=\tp/(\tp+\fp), which is also \tpr.

For DP, we use a clipping bound $C=1$, $\delta=1e-5$, and vary the noise scale $\sigma$. Privacy bound $\epsilon$ is accumulated using  moments accountant~\cite{abadi2016deep}. The larger $\sigma$ is, the more noise is applied, and the smaller the $\epsilon$, indicating the 
%tighter the privacy bound. 
better the privacy.
For all experiment settings including the baseline model DeepLog, we train a LSTM model for 100 epochs, and use the final model as the anomaly detection model. The model related parameters are: 2 layers, 256 units per layer, 10 time steps, and a batch size of 256.

\paragraph{Probability-based detection.}
As a preliminary result, we use probability-based anomaly detection to demonstrate the effectiveness of DP noise in reducing \fn. Table~\ref{table:prob} shows \fn and \fp for DeepLog and DeepLog+DP with increasing noise levels, under different probability thresholds $T_p$. It is clear that DP noise could effectively reduce \fn, and the larger noise being added, the more false negatives are reduced. We also note that when $\sigma=0.25$, the privacy bound $\epsilon=90.5$. It is often thought that a DP bound $\epsilon>20$ is completely useless in terms of protecting privacy. Here we indicate that a small amount of noise may be enough to reduce \fn. Although more false positives are incurred because of DP noise, the drop in \tpr is negligible, considering the large volume of normal data. For example, when $T_p=2e-6$ and $\sigma=1$, the \fn drop from 1261 to 183 indicates a \tnr increase of 8\% ($91.7\% \to 98.8\%$), while the \fp increase from 2291 to 3734 only shows a \tpr decrease of 0.3\% ($99.59\% \to 99.32\%$).

\begin{table}[hbt]
\vspace{-1mm}
	\centering
	\small
	\caption{{Probability-based anomaly detection results}. }
	\label{table:prob}
	\tabcolsep=0.12cm
    \begin{tabular}{ |l|r|r|r|r|r| } \hline
    Threshold & {DeepLog}  &  \multicolumn{4}{|c|}{DeepLog+DP (\fn/\fp)}  \\  \cline{3-6}
    {$T_p$}    & \fn/\fp & $\sigma=0.25$ & $\sigma=1$ & $\sigma=1.5$ & $\sigma=2$   \\ \hline
%    $1e-4$  & 89/5855 &  1/19614 & 0/13672 & 0/25080  &  1/22967   \\ \hline
    $1e-5$  &   573/3596  &  7/14268 & 0/6059 &1/8213   &   1/9187   \\ \hline
    $2e-6$  &  1261/2291 & 208/4756  & 183/3734 &1/5718   &  1/6317 \\ \hline
    $1e-6$  &  1468/2068 & 410/3759 & 190/3552 & 2/4002   &  1/6093 \\ \hline
    \end{tabular}
\end{table}

\begin{figure}[b!]
	\centering{
		\includegraphics[width=\linewidth]{fpfn_crop.pdf}
	}
	\vspace{-2mm}
	\caption{Comparison of \fp and \fn.}
	\label{fig:fpfn}
\end{figure}
\begin{figure}[h!]
	\centering{
		\includegraphics[width=\linewidth]{fm_crop.pdf}
	}
	\vspace{-2mm}
	\caption{Comparison of \fm (horizontal lines: DeepLog).}
	\label{fig:fm}
\end{figure}


% 'deeplog': 0.9992558587410864, 
% 'deeplog_sigma0.25': 0.9997235282443324, 
% 'deeplog_sigma0.5': 0.9996685355610535, 
% 'deeplog_sigma0.75': 0.9997040718392682, 
% 'deeplog_sigma1.0': 0.9998035320746803, 
% 'deeplog_sigma1.25': 0.9993137656954586}
% auc {'deeplog_sigma1.5': 0.9993796980162404, 
% 'deeplog_sigma1.75': 0.9989275235575203, 
% 'deeplog_sigma2.0': 0.9984938573726088, 
\begin{table*}[htb]
	\centering
	\caption{{AUC score comparison and DP bound $\epsilon$}. }
	\label{table:auc}
%	\tabcolsep=0.12cm
    \begin{tabular}{ |l|r|r|r|r|r|r|r|r|r| } \hline
     & \multirow{ 2}{*}{DeepLog}  &  \multicolumn{8}{|c|}{DeepLog+DP}  \\  \cline{3-10}
     &  & $\sigma$=$0.25$ & $\sigma$=$0.5$ & $\sigma$=$0.75$ & $\sigma$=$1.0$ & $\sigma$=$1.25$ & $\sigma$=$1.5$ & $\sigma$=$1.75$  & $\sigma$=$2.0$   \\ \hline
    \auc score & 0.9993   & 0.9997  & 0.9997 & 0.9997  & 0.9998 & 0.9993  & 0.9994 & 0.9989 & 0.9985 \\ \hline
    DP bound $\epsilon$ & 0  & 90.45  & 6.21 & 1.86   &  0.96 & 0.61 & 0.42 & 0.31 & 0.25 \\ \hline
    \end{tabular}
\end{table*}

% 'results_sample1_non_dp_epoch100_validLoss0.236_validAcc91.11_eps0_delta1e-05_sigma2.0_clip1.0' , \
% 'results_sample1_dp_clip1.0_delta1e-05_sigma0.25_clip1.0_epoch100_validLoss0.520_validAcc90.64_eps90.4542736127', 
% 'results_sample1_dp_clip1.0_delta1e-05_sigma0.5_clip1.0_epoch100_validLoss0.472_validAcc90.55_eps6.20790357135', 
% 'results_sample1_dp_clip1.0_delta1e-05_sigma0.75_epoch100_validLoss0.525_validAcc89.01_eps1.85659161702', 
% 'results_sample1_dp_clip1.0_delta1e-05_epoch100_validLoss0.507_validAcc88.11_eps0.9585177585005272_delta1e-05_sigma1.0_clip1.0', \
% 'results_sample1_dp_clip1.0_delta1e-05_sigma1.25_clip1.0_epoch100_validLoss0.514_validAcc87.85_eps0.6058708360081059', \
% 'results_sample1_dp_clip1.0_delta1e-05_sigma1.5_clip1.0_epoch100_validLoss0.515_validAcc87.55_eps0.421239796147']
% 'results_sample1_dp_clip1.0_delta1e-05_sigma1.75_clip1.0_epoch100_validLoss0.513_validAcc87.51_eps0.3147356032840113', \
% 'results_sample1_dp_clip1.0_delta1e-05_epoch100_validLoss0.515_validAcc87.20_eps0.2495376875746713_delta1e-05_sigma2.0_clip1.0', \

%\section{Applying differential privacy (DP) to out-of-distribution (OOD) detection}


\paragraph{Topk-based detection.}
Nevertheless, as used in DeepLog, we find that {topk-based} detection criteria result in much better overall \fm for both DeepLog and DeepLog+DP. So next we focus on this detection method, to comprehensively evaluate the effect of applying DP noise to anomaly detection.
Figure~\ref{fig:fpfn} shows the comparison of \fp and \fn under different thresholds $k$, with the increase of noise scale $\sigma$. For clarity, we only show the following two cases for baseline model DeepLog: k=10 which has the maximum \fp and the minimum \fn, and k=18 which has the minimum \fp and the maximum \fn. Note that y axis is plotted as log scale.
It is clear that applying DP noise significantly reduces \fn in all cases, from over a thousand in DeepLog, to hundreds or even zero in DeepLog+DP. Also, the larger noise being added, the more \fn are reduced, while the more \fp are introduced, which emphasizes our observation in previous {probability-based} detection method.


%To evaluate the overall performance of DeepLog+DP compared with DeepLog under different thresholds,
The \fm measurements are plotted in Figure~\ref{fig:fm}. For DeepLog model, \fm ranges from 90.38\% (k=20) to 93.81\% (k=10). 
For DeepLog+DP, the best \fm scores include 96.29\% ($\sigma=0.25$, $k=15$) and 96.28\% ($\sigma=1$, $k=18$), which show clear improvements over DeepLog model. As shown in the figure, DeepLog performs better when $k$ is smaller, while DeepLog+DP benefits from larger $k$s. This scenario could also be explained by the addition of DP noise. Since the trained model does not overfit to outliers, it assigns to anomalies much lower probabilities, which are consequently ranked much lower than in the DeepLog model. Meanwhile, normal execution logs are also possibly predicted with lower probabilities because of the uncertainty brought by DP noise. As a result, the ideal threshold $k$ for DeepLog+DP is higher than that of DeepLog. We also note that a large noise scale could hurt the overall performance, as shown by the downward trend when $\sigma$ increases from $1.75$ to $2.0$.


%To evaluate the overall performance under different thresholds $k$, 
To evaluate the overall performance of DeepLog+DP compared with DeepLog under different thresholds,
we further compute the \auc score of DeepLog and DeepLog+DP with different noise scale $\sigma$.
\auc stands for \textit{Area under curve (\auc) score}, which is the area under 
\textit{receiver operating characteristic (ROC) curve}, where the x axis is the \fpr while the y axis denotes the \tpr. Clearly, the lower the \fpr and the higher the \tpr, the bigger the area under ROC curve, and hence the larger the \auc score.
As shown in Table~\ref{table:auc}, DeepLog already achieves excellent \auc score, considering the large amount of normal data and the significantly fewer anomalies. However, an adequate amount of DP noise is still able to improve the performance. 

Table~\ref{table:auc} also indicates the privacy bound $\epsilon$. Note that $\epsilon<10$ is often considered as usable and $\epsilon<1$ is a tight bound that well protects privacy. Considering all the cases, $\sigma=1$ gives the best anomaly detection utility as well as a tight privacy bound to protect training data privacy.


\section{Discussion}
Adding DP noise to DeepLog significantly reduces the number of false negatives and further improves the overall performance. Although it is often accompanied with more false positives, we note that in system anomaly detection, the merit of fewer false negatives in fact worth the cost of more false positives. That is because reported false positives could be further checked by system admin, and then fed into the model for incremental learning. However, a false negative may never be found out, until a more disastrous event occurs due to the un-discovery of it.

We also note that a set of recent work for out-of-distribution (OOD) detection~\cite{hendrycks2016baseline, hendrycks2018deep} also train a detection model without knowing the positives to detect. It would be interesting to explore whether the addition of DP noise could help to improve OOD detection results, or reduce the number of false negatives. We plan to explore this as our future work.


\section{Conclusion}
\vspace{-1mm}
In this paper, we leverage the fact that differential privacy (DP) helps to prevent overfitting in deep learning model training, and apply DP noise to a zero-positive anomaly detection model, DeepLog. The evaluation results show that DP noise is effective towards reducing the number of false negatives, and further improving the overall utility. 
% In terms of differential privacy, we show that although a small amount of noise may not be helpful in protecting user privacy, it has the merit of improving anomaly detection performance.
In the meantime, the tight privacy bound provided by DP noise also helps with protecting training data privacy.





%%%%%%%%%%%%%%%%%% bk %%%%%%%%%%%%%%%%%%%%%%%%%
SKETCH: (DP $\rightarrow$ low generalization error $\rightarrow$ $f$ closer to true distribution $\rightarrow$ outlier is easier to be detected)

\begin{enumerate}
    \item Suppose there are $n$ training instances in the training dataset $\mathcal{D}$. Generalization error $Err_{gen}$ measures how close the result summarized from $\mathcal{D}$ is to the result summarized from its true distribution $\mathbb{D}$:
    \begin{equation}
    \label{sec:ge_err}
        Err_{gen} = \mathbb{E}_{z\sim\mathbb{D}} [f(z)] - \frac{1}{n} \sum_{z\in \mathcal{D}} f(z)
    \end{equation}
    
    \item Previous statistical results show that differential privacy implies low generalization error. Specifically, in Theorem 7.2 of \cite{bassily2016algorithmic}:
    \begin{equation}
    \label{eq:dp_err}
        P[||f_{(\epsilon, \delta)}(\mathbb{D}) - f_{(\epsilon, \delta)}(\mathcal{D})|| \ge 18 \epsilon \Delta n] < \frac{\delta}{\epsilon}
    \end{equation}

    \item The following shows that, dp ensures with high probability, $z_o$ could be detected by the model learned from $\mathcal{D}$.
    \begin{align*}
    \label{eq:err_D}
        ||f_{(\epsilon, \delta)}(d) - f_{(\epsilon, \delta)}(\mathcal{D})|| 
        &= ||f_{(\epsilon, \delta)}(d) - f_{(\epsilon, \delta)}(\mathbb{D}) + f_{(\epsilon, \delta)}(\mathbb{D}) - f_{(\epsilon, \delta)}(\mathcal{D})|| \\
        &\ge ||f_{(\epsilon, \delta)}(d) - f_{(\epsilon, \delta)}(\mathbb{D})|| - ||f_{(\epsilon, \delta)}(\mathbb{D}) - f_{(\epsilon, \delta)}(\mathcal{D})|| \\
        &\ge T - ||f_{(\epsilon, \delta)}(\mathbb{D}) - f_{(\epsilon, \delta)}(\mathcal{D})||
    \end{align*}
    Combining Equation \ref{eq:dp_err}, we have:
    \begin{equation}
    \label{eq:p_err_D}
        P[||f_{(\epsilon, \delta)}(z_o) - f_{(\epsilon, \delta)}(\mathcal{D})|| \ge  T- 18 \epsilon \Delta n  ] \ge 1- \frac{\delta}{\epsilon}
    \end{equation}    
    
\end{enumerate}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mind{thinking of combing the two tables together and show AUPR only.}

\begin{table}[hbt]
\vspace{-1mm}
	\centering
	\small
	\caption{{AUPR/AUROC score of training data}. }
	\label{table:train_ae}
	\tabcolsep=0.12cm
    \begin{tabular}{ |l|r|r|r|r|r|r| } \hline
    noise   &  \multicolumn{6}{|c|}{outlier percentage in training data $r_o$}  \\  \cline{2-7}
    scale    &  $10^{-4}$ & $10^{-3}$ & $5 \times 10^{-3}$ & $10^{-2}$ & $5 \times 10^{-2}$ & $10^{-1}$   \\ \hline
    $\sigma=0$  &   
100/100 &
99.92/100.0 &
92.12/99.81 &
92.12/99.81 &
84.33/97.3 &
72.16/89.46
   \\ \hline

    $\sigma=10^{-3}$  &  
                        &
100/100 &
98.37/99.89 &
94.33/99.79 &
84.31/97.37 &
86.51/96.26 
 \\ \hline

    $\sigma=5 \times 10^{-3}$  &  
                        &
i2                      &
98.69/99.92  &
g3                      &
g3                      &
c1
 \\ \hline
    $\sigma=10^{-2}$  &  
                        &
100/100 &
94.92/99.8  &
97.08/99.89  &
90.79/98.39  &
85.41/96.02
 \\ \hline
    $\sigma=5 \times 10^{-2}$  &  
                        &
i2                      &
97.97/99.9   &
g2                      &
g2                      &
c1      
 \\ \hline
    $\sigma=10^{-1}$  &  
                        &
100/100 &
98.44/99.87 &
93.11/99.58 &
92.23/98.77                     &
85.56/96.16 
 \\ \hline
    $\sigma=5 \times 10^{-1}$  &  
& & & & & \\ \hline
    $\sigma=1$  &  
                        &
100/100 &
98.28/99.91 &
95.8/99.74   &
94.92/99.31 &
81.87/94.66 
\\ \hline
    $\sigma=5$  &  
                        &
i2                      &
98.51/99.96 &
96.5/99.52   &
96.78/99.07 &
95.25/98.49
\\ \hline
    $\sigma=10$  &  
                &
c0                  &
91.88/99.14  &
97.5/99.68  &
96.6/98.722  &
97.07/98.9  
\\ \hline
    $\sigma=50$  &  
c3 &
c0 &
c2 &
c2 &
c3 &
c1
\\ \hline
    $\sigma=100$  &  
 &
 &
 &
 &
 &

\\ \hline
    \end{tabular}
\end{table}




\begin{table}[hbt]
\vspace{-1mm}
	\centering
	\small
	\caption{{AUPR/AUROC score of test data}. }
	\label{table:test_ae}
	\tabcolsep=0.12cm
    \begin{tabular}{ |l|r|r|r|r|r|r| } \hline
    noise   &  \multicolumn{6}{|c|}{outlier percentage in training data $r_o$}  \\  \cline{2-7}
    scale    &  $10^{-4}$ & $10^{-3}$ & $5 \times 10^{-3}$ & $10^{-2}$ & $5 \times 10^{-2}$ & $10^{-1}$   \\ \hline
    $\sigma=0$  &   
99.84/99.97 &
99.77/99.95 &
98.81/99.79 &
98.81/99.79 &
88.18/97.4 &
68.14/89.2
   \\ \hline

    $\sigma=10^{-3}$  &  
                        &
99.86/99.97 &
99.64/99.93 &
98.81/99.82 &
89.34/97.63 &
85.58/96.72 
 \\ \hline

    $\sigma=5 \times 10^{-3}$  &  
                        &
i2                      &
99.7/99.93  &
g3                      &
g3                      &
c1
 \\ \hline
    $\sigma=10^{-2}$  &  
                        &
99.97 &
99.23/99.87  &
99.33/99.9  &
93.34/98.5  &
84.07/96.4
 \\ \hline
    $\sigma=5 \times 10^{-2}$  &  
                        &
i2                      &
99.55/99.9   &
g2                      &
g2                      &
c1      
 \\ \hline
    $\sigma=10^{-1}$  &  
                        &
99.85/99.97 &
99.66/99.94 &
98.21/99.71 &
94.21/98.82      &
83.98/96.46 
 \\ \hline
    $\sigma=5 \times 10^{-1}$  &  
& & & & & \\ \hline
    $\sigma=1$  &  
                        &
99.78/99.94 &
99.67/99.91 &
99.0/99.81   &
96.87/99.44 &
80.12/94.95 
\\ \hline
    $\sigma=5$  &  
                        &
i2                      &
99.52/99.84 &
98.78/99.5   &
98.04/99.32 &
95.41/98.74
\\ \hline
    $\sigma=10$  &  
                &
c0                  &
98.2/99.22  &
99.12/99.79  &
98.2/99.29  &
97.46/99.27  
\\ \hline
    $\sigma=50$  &  
c3 &
c0 &
c2 &
c2 &
c3 &
c1
\\ \hline
    $\sigma=100$  &  
 &
 &
 &
 &
 &

\\ \hline
    \end{tabular}
\end{table}
